Towards Infinite-Long Prefix in Transformer

Prompting and context-based fine-tuning methods, which we call Prefix Learning, have been proposed to enhance the performance of language models on various downstream tasks. They are empirically efficient and effective, matching the performance of full parameter fine-tuning, but the theoretical understandings are limited. In this paper, we aim to address this limitation by studying their ability from the perspective of prefix length. In particular, we provide a convergence guarantee for training an ultra-long prefix in a stylized setting using the Neural Tangent Kernel (NTK) framework. Based on this strong theoretical guarantee, we design and implement an algorithm that only needs to introduce and fine-tune a few extra trainable parameters instead of an infinite-long prefix in each layer of a transformer, and can approximate the prefix attention to a guaranteed polynomial-small error. Preliminary experimental results on vision, natural language, and math data show that our method achieves superior or competitive performance compared to existing methods like full parameters fine-tuning, P-Tuning V2, and LoRA. This demonstrates our method is promising for parameter-efficient fine-tuning. Our code can be found at \url{https://github.com/ChristianYang37/chiwun/tree/main/src/NTK-Attention}.

==> 18_app_gradeint_more.tex <==
\section{Gradient Computation}\label{sec:more_gradient_computation}
In this section, we provide additional gradient computation for our NTK-Attention.
\subsection{Gradient of \texorpdfstring{$f(x, P)$}{}}

\begin{lemma}
    Let function $f:\R^d \times \R^{n \times d} \rightarrow \R^d$ be defined as Definition~\ref{def:f_x}, for a vector $x \in \R^d$ and an matrix $P \in \R^{m \times d}$, we have
    \begin{align*}
        \frac{\d}{\d P_s} f(x, P) = s(x, P_s) \frac{ (v(P_s) - f(x, P)) \cdot W_{qk}^\top x + w_v }{\sum_{r=1}^m s(x, P_r) + s(x, x)}
    \end{align*}
\end{lemma}

\begin{proof}
    We have
    \begin{align*}
        \frac{\d}{\d P_s} f(x, P)
        = & ~ \frac{\d}{\d P_s} \frac{\sum_{r=1}^m s(x, P_r) v(P_r) + s(x, x) v(x)}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \\
        = & ~ \frac{1}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \cdot \frac{\d}{\d P_s} ( \sum_{r=1}^m s(x, P_r) v(P_r) ) \\
        & ~ + (\sum_{r=1}^m s(x, P_r) v(P_r) + s(x, x) v(x)) \cdot \frac{\d}{\d P_s} \frac{1}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \\
        = & ~ \frac{1}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \cdot \frac{\d}{\d P_s} ( s(x, P_s) v(P_s) ) \\
        & ~ + (\sum_{r=1}^m s(x, P_r) v(P_r) + s(x, x) v(x)) \cdot \frac{\d}{\d P_s} \frac{1}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \\
        = & ~ \frac{1}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \cdot (v(P_s) \frac{\d}{\d P_s}  s(x, P_s) + s(x, P_s) \frac{\d}{\d P_s} v(P_s) ) \\
        & ~ + (\sum_{r=1}^m s(x, P_r) v(P_r) + s(x, x) v(x)) \cdot \frac{\d}{\d P_s} \frac{1}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \\
        = & ~ \frac{1}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \cdot (v(P_s) \frac{\d}{\d P_s}  s(x, P_s) + s(x, P_s) \frac{\d}{\d P_s} v(P_s) ) \\
        & ~ - (\sum_{r=1}^m s(x, P_r) v(P_r) + s(x, x) v(x)) \cdot \frac{1}{(\sum_{r=1}^m s(x, P_r) + s(x, x))^2} \frac{\d}{\d P_s} s(x, P_s) \\
        = & ~ \frac{ v(P_s) s(x, P_s)\cdot W_{qk}^\top x + s(x, P_s) \cdot w_v }{\sum_{r=1}^m s(x, P_r) + s(x, x)} \\
        & ~ - (\sum_{r=1}^m s(x, P_r) v(P_r) + s(x, x) v(x)) \cdot \frac{s(x, P_s)\cdot W_{qk}^\top x}{(\sum_{r=1}^m s(x, P_r) + s(x, x))^2} \\
        = & ~ \frac{ v(P_s) s(x, P_s)\cdot W_{qk}^\top x + s(x, P_s) \cdot w_v }{\sum_{r=1}^m s(x, P_r) + s(x, x)} - f(x, P) \cdot \frac{s(x, P_s)\cdot W_{qk}^\top x}{\sum_{r=1}^m s(x, P_r) + s(x, x)} \\
        = & ~ s(x, P_s) \frac{ (v(P_s) - f(x, P)) \cdot W_{qk}^\top x + w_v }{\sum_{r=1}^m s(x, P_r) + s(x, x)}
    \end{align*}
    where the first step follows from Definition~\ref{def:f_x}, the second step follows from chain rules, the third step follows from $\frac{\d}{\d P_s} s(x, P_r) = 0$ for $s \ne r$, the fourth and fifth steps follow from chain rules, the sixth step follows from Lemma~\ref{lem:grad_s} and Lemma~\ref{lem:grad_v}, the seventh step follows from Definition~\ref{def:f_x} and the last step follows from simple algebra.
\end{proof}

\subsection{Gradient of \texorpdfstring{$s(x, P_r)$}{}}

\begin{lemma}\label{lem:grad_s}
    Let function $s:\R^d \times \R^{ d} \rightarrow \R^d$ be defined as Definition~\ref{def:s}, for a vector $x \in \R^d$ and an matrix $P \in \R^{m \times d}$, we have
    \begin{align*}
        \frac{\d}{\d P_r} s(x, P_r) = s(x, P_r) W_{qk}^\top x
    \end{align*}
\end{lemma}

\begin{proof}
    We have
    \begin{align*}
        \frac{\d}{\d P_r} s(x, P_r)
        = & ~ \frac{\d}{\d P_r} \exp(x^\top W_{qk}P_r) \\
        = & ~ \exp(x^\top W_{qk}P_r) \frac{\d}{\d P_r} x^\top W_{qk}P_r \\
        = & ~ \exp(x^\top W_{qk}P_r) W_{qk}^\top x \\
        = & ~ s(x, P_r) W_{qk}^\top x
    \end{align*}
    where the first step follows from Definition~\ref{def:s}, the second step follows from chain rules, the third step follows from differential rule and the last step follows from Definition~\ref{def:s}.
\end{proof}

\subsection{Gradient of \texorpdfstring{$v(x)$}{}}

\begin{lemma}\label{lem:grad_v}
    Let function $v:\R^d \rightarrow \R$ be defined as Definition~\ref{def:v_x}, for a vector $x \in \R^d$, we have
    \begin{align*}
        \frac{\d}{\d P_r} v(P_r) = w_v
    \end{align*}
\end{lemma}

\begin{proof}
    We have
    \begin{align*}
        \frac{\d}{\d P_r} v(P_r)
        = & ~ \frac{\d}{\d P_r} \langle P_r, w_v \rangle \\
        = &  ~ w_v
    \end{align*}
    where the first step follows from Definition~\ref{def:v_x}, the second step follows from simple differential rules.
\end{proof}
